Kicking it Off(-shell) with Direct Diffusion

Off-shell effects in large LHC backgrounds are crucial for precision predictions and, at the same time, challenging to simulate. We present a novel method to transform high-dimensional distributions based on a diffusion neural network and use it to generate a process with off-shell kinematics from the much simpler on-shell one. Applied to a toy example of top pair production at LO we show how our method generates off-shell configurations fast and precisely, while reproducing even challenging on-shell features.

==> incl_comments.tex <==
%\usepackage{xcolor}
%\usepackage{ulem}
\definecolor{darkgreen}{rgb}{0,0.4,0}
\newcommand{\commentTJ}[1]{\textcolor{orange}{(TJ: #1)}}
\newcommand{\addedTJ}[1]{\textcolor{orange}{#1}}
\newcommand{\deletedTJ}[1]{\sout{\textcolor{orange}{#1}}}
